Vision-based Multi-future Trajectory Prediction: A Survey

Vision-based trajectory prediction is an important task that supports safe and intelligent behaviours in autonomous systems. Many advanced approaches have been proposed over the years with improved spatial and temporal feature extraction. However, human behaviour is naturally diverse and uncertain. Given the past trajectory and surrounding environment information, an agent can have multiple plausible trajectories in the future. To tackle this problem, an essential task named multi-future trajectory prediction (MTP) has recently been studied. This task aims to generate a diverse, acceptable and explainable distribution of future predictions for each agent. In this paper, we present the first survey for MTP with our unique taxonomies and a comprehensive analysis of frameworks, datasets and evaluation metrics. We also compare models on existing MTP datasets and conduct experiments on the ForkingPath dataset. Finally, we discuss multiple future directions that can help researchers develop novel multi-future trajectory prediction systems and other diverse learning tasks similar to MTP.

==> figures/datasets.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[trim={2cm 0 0 0},clip,width=0.8\textwidth]{figures/datasets/sdd.png}
         \caption{SDD}
         \label{fig:noise-injection}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figures/datasets/nuscenes.png}
         \caption{Vehicle TP Benchmarks}
         \label{fig:noise-injection}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figures/datasets/virat.png}
         \caption{VIRAT}
         \label{fig:noise-injection}
     \end{subfigure}
     
    \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figures/datasets/multipath.png}
         \caption{MultiPath Toy Dataset}
         \label{fig:noise-injection}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figures/datasets/social-ways.jpeg}
         \caption{6-way Toy Dataset}
         \label{fig:noise-injection}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figures/datasets/forkingpath.jpeg}
         \caption{Forking Path}
         \label{fig:noise-injection}
     \end{subfigure}

     \caption{Example of MTP datasets.}
     \label{fig:mtp_datasets}
\end{figure*}

==> tab/all_equations.tex <==


\begin{table*}[t]
    \centering
    \scalebox{1}{
    \begin{tabular}{c|p{0.15\textwidth}|l|p{0.20\textwidth}} 
    \toprule
    ~ & Loss & Equation & Description\\ \midrule
    
    \multirow{3}{*}{\rotatebox[origin=c]{-90}{\parbox[c]{3cm}{\centering \small{Lower Bound based}}}} &

    Minimum-of-N & 
    \(
    MoN= \mathbb{E}_{i,t\in \tau} \min_{k<K} DE(\hat{Y}_{i,k}^t, Y_{i}^t) 
    \) &
    The ``best'' results among $K$ future predictions and wraps an existing evaluation metric $DE$  
    \\\cmidrule{2-4}
    
    & Missing/Hit rate & 
    \( R = \mathbb{E}_{i,t\in \tau} 
    \begin{cases}
      \textbf{Missing: }(\min_{k<K} FDE(\hat{Y}_{i,k}^t, Y_{i}^t)) > d  \\
    \textbf{Hit: } (\min_{k<K} FDE(\hat{Y}_{i,k}^t, Y_{i}^t)) \le d
    \end{cases}
    \)
    &
    The best score among $K$ predicted trajectories.
    \\\midrule

    & mAP & 
    \begin{tabular}[c]{@{}p{0.4\textwidth}@{}}
        \(
            mAP(\hat{Y}_{i,k'}^t) =  \frac{ \sum_{i<N} \textbf{Hit}}
            {(\sum_{i<N} \textbf{Hit} * \sum_{i<N} \textbf{Missing})}
        \) \\
       \centering
        \(\text{where }  \hat{Y}_{i,k*}^\tau = \arg \max_k \mathcal{P}(\hat{Y}_{i,k}^\tau)\)

    \end{tabular}&
    The best score among $K$ predicted trajectories.
    \\\cmidrule{2-4}

    \multirow{4}{*}{\rotatebox[origin=c]{-90}{\parbox[c]{4cm}{\centering \small Distribution-based}}} &

    KDE-NLL & 
    \(
    \text{KDE-NLL} = - \mathbf{E}_{i,t} \log \text{KDE}(\hat{Y}_{i,K}^t, Y_{i}^t)
    \) &
    The best score among $K$ predicted trajectories.
    \\\cmidrule{2-4}
    
    & Recall and Precision for Generative Network & 
    \begin{tabular}[c]{@{}p{0.4\textwidth}@{}}
    \centering
        \(
        Recall(\hat{Y}_i^t, Y_i^t) = \mathbb{E}_{K_G} (\min_{k'< K_R} || \hat{Y}_{i,k}^t - Y_{i,k'}^t ||_2 ) < d 
        \) \\
        \(
        Precision(\hat{Y}_i^t, Y_i^t) = \mathbb{E}_{K_R} (\min_{k'< K_G} || Y_{i,k}^t - \hat{Y}_{i,k'}^t ||_2 ) < d 
        \) \\
        \raggedright
        \textbf{Note: $K_R$ and $K_G$ are the numbers of trajectories in predictions and ground truth are not required to be equal.}
    \end{tabular}
    & \small{The coverage between the annotated ground truth and predicted distribution. }
    \\\cmidrule{2-4}


    & PCMD & 
    \(\text{PCMD} = \mathbb{E}_{i,t} \min(DE(i), \mathcal{P} (\hat{Y}_{i,k} | X_i^T) \ge \gamma)\)
    &
    The best score among $K$ predicted trajectories.
    \\\cmidrule{2-4}

    & AMD / AMV & 
    \begin{tabular}[c]{@{}p{0.40\textwidth}@{}}
        \(
        AMD = \mathbf{E}_{i,t\in \tau} \sqrt{(\mu_i^\tau - Y_i^\tau)^T \hat{G}(\mu_i^\tau - Y_i^\tau)}
        \) \\
        \(
        AMV = \mathbf{E}_{i,t\in \tau} Eigenvalue(\Sigma_i^\tau)
        \)
    \end{tabular}
    &
    The best score among $K$ predicted trajectories.
    \\\bottomrule
    
    \end{tabular}
    }
    \caption{A table for evaluation metrics. Under modification now}
    \label{tab:metrics}
\end{table*}

==> tab/evaluation_metrics_table.tex <==


\begin{table*}[t]
    \centering
    \scalebox{1}{
    \begin{tabular}{c|p{0.15\textwidth}|l|p{0.20\textwidth}} 
    \toprule
    ~ & Loss &  Description & \\ \midrule
    
    \multirow{3}{*}{\rotatebox[origin=c]{-90}{\parbox[c]{3cm}{\centering \small{Lower Bound based}}}} &

    Minimum-of-N & 
    \(
    MoN= \mathbb{E}_{i,t\in \tau} \min_{k<K} DE(\hat{Y}_{i,k}^t, Y_{i}^t) 
    \) &
    The ``best'' results among $K$ future predictions and wraps an existing evaluation metric $DE$  
    \\\cmidrule{2-4}
    
    & Missing/Hit rate & 
    \( R = \mathbb{E}_{i,t\in \tau} 
    \begin{cases}
      \textbf{Missing: }(\min_{k<K} FDE(\hat{Y}_{i,k}^t, Y_{i}^t)) > d  \\
    \textbf{Hit: } (\min_{k<K} FDE(\hat{Y}_{i,k}^t, Y_{i}^t)) \le d
    \end{cases}
    \)
    &
    The best score among $K$ predicted trajectories.
    \\\midrule

    & mAP & 
    \begin{tabular}[c]{@{}p{0.4\textwidth}@{}}
        \(
            mAP(\hat{Y}_{i,k'}^t) =  \frac{ \sum_{i<N} \textbf{Hit}}
            {(\sum_{i<N} \textbf{Hit} * \sum_{i<N} \textbf{Missing})}
        \) \\
       \centering
        \(\text{where }  \hat{Y}_{i,k*}^\tau = \arg \max_k \mathcal{P}(\hat{Y}_{i,k}^\tau)\)

    \end{tabular}&
    The best score among $K$ predicted trajectories.
    \\\cmidrule{2-4}

    \multirow{4}{*}{\rotatebox[origin=c]{-90}{\parbox[c]{4cm}{\centering \small Distribution-based}}} &

    KDE-NLL & 
    \(
    \text{KDE-NLL} = - \mathbf{E}_{i,t} \log \text{KDE}(\hat{Y}_{i,K}^t, Y_{i}^t)
    \) &
    The best score among $K$ predicted trajectories.
    \\\cmidrule{2-4}
    
    & Recall and Precision for Generative Network & 
    \begin{tabular}[c]{@{}p{0.4\textwidth}@{}}
    \centering
        \(
        Recall(\hat{Y}_i^t, Y_i^t) = \mathbb{E}_{K_G} (\min_{k'< K_R} || \hat{Y}_{i,k}^t - Y_{i,k'}^t ||_2 ) < d 
        \) \\
        \(
        Precision(\hat{Y}_i^t, Y_i^t) = \mathbb{E}_{K_R} (\min_{k'< K_G} || Y_{i,k}^t - \hat{Y}_{i,k'}^t ||_2 ) < d 
        \) \\
        \raggedright
        \textbf{Note: $K_R$ and $K_G$ are the numbers of trajectories in predictions and ground truth are not required to be equal.}
    \end{tabular}
    & \small{The coverage between the annotated ground truth and predicted distribution. }
    \\\cmidrule{2-4}


    & PCMD & 
    \(\text{PCMD} = \mathbb{E}_{i,t} \min(DE(i), \mathcal{P} (\hat{Y}_{i,k} | X_i^T) \ge \gamma)\)
    &
    The best score among $K$ predicted trajectories.
    \\\cmidrule{2-4}

    & AMD / AMV & 
    \begin{tabular}[c]{@{}p{0.40\textwidth}@{}}
        \(
        AMD = \mathbf{E}_{i,t\in \tau} \sqrt{(\mu_i^\tau - Y_i^\tau)^T \hat{G}(\mu_i^\tau - Y_i^\tau)}
        \) \\
        \(
        AMV = \mathbf{E}_{i,t\in \tau} Eigenvalue(\Sigma_i^\tau)
        \)
    \end{tabular}
    &
    The best score among $K$ predicted trajectories.
    \\\bottomrule
    
    \end{tabular}
    }
    \caption{A table for evaluation metrics. Under modification now}
    \label{tab:metrics}
\end{table*}
